D4M 3.0: Extended Database and Language Capabilities

The D4M tool was developed to address many of today's data needs. This tool is used by hundreds of researchers to perform complex analytics on unstructured data. Over the past few years, the D4M toolbox has evolved to support connectivity with a variety of new database engines, including SciDB. D4M-Graphulo provides the ability to do graph analytics in the Apache Accumulo database. Finally, an implementation using the Julia programming language is also now available. In this article, we describe some of our latest additions to the D4M toolbox and our upcoming D4M 3.0 release. We show through benchmarking and scaling results that we can achieve fast SciDB ingest using the D4M-SciDB connector, that using Graphulo can enable graph algorithms on scales that can be memory limited, and that the Julia implementation of D4M achieves comparable performance or exceeds that of the existing MATLAB(R) implementation.

==> makefile <==
BUILD := \
	D4M_HPEC_2017

DEPS := \
	D4M_HPEC_2017.bib

LATEX  := latex
BIBTEX := bibtex
DVIPS  := dvips
PS2PDF := ps2pdf

RM      := rm
RMFLAGS := -rf

TARGETS := $(patsubst %, %.pdf, $(BUILD))

%.dvi: %.tex %.bib $(DEPS)
	$(eval SRC_$@ = $(patsubst %.tex, %, $<))
	$(LATEX) $(SRC_$@)
	$(BIBTEX) $(SRC_$@)
	$(LATEX) $(SRC_$@)
	$(LATEX) $(SRC_$@)

%.ps: %.dvi
	$(eval SRC_$@ = $(patsubst %.tex, %, $<))
	$(DVIPS) $(SRC_$@)

%.pdf: %.ps
	$(PS2PDF) $<

all: $(TARGETS)

clean:
	$(RM) $(RMFLAGS) *.aux *.log *.blg *.bbl *.ent *.out *.dvi *.ps *.pdf

.PHONY: all clean

